Automating Proofs of Data-Structure Properties in Imperative Programs

We consider the problem of automated reasoning about dynamically manipulated data structures. The state-of-the-art methods are limited to the unfold-and-match (U+M) paradigm, where predicates are transformed via (un)folding operations induced from their definitions before being treated as uninterpreted. However, proof obligations from verifying programs with iterative loops and multiple function calls often do not succumb to this paradigm. Our contribution is a proof method which -- beyond U+M -- performs automatic formula re-writing by treating previously encountered obligations in each proof path as possible induction hypotheses. This enables us, for the first time, to systematically reason about a wide range of obligations, arising from practical program verification. We demonstrate the power of our proof rules on commonly used lemmas, thereby close the remaining gaps in existing state-of-the-art systems. Another impact, probably more important, is that our method regains the power of compositional reasoning, and shows that the usage of user-provided lemmas is no longer needed for the existing set of benchmarks. This not only removes the burden of coming up with the appropriate lemmas, but also significantly boosts up the verification process, since lemma applications, coupled with unfolding, often induce very large search space.

==> algo.tex <==


\begin{figure}[tbh]
\begin{center}
\small{
$\begin{array}{rl}

\multicolumn{2}{l}{\mbox{\bf function} ~\func{Prove}(\Left \models \Right, ~\tilde{A}, ~lb, ~rb, ~ib)}  \\
%\ppp & \pair{Obs}{success} ~\Assign ~\func{partition}(\Left \models \Right, \tilde{A}, lb, rb , ib) \\
%\ppp & \If ~(success) ~\Return ~\func{ProveAll}(Obs) \\
%\\

     & \mbox{/* Natural proof, i.e. by unification and \smt{} */} \\
\ppp & \If ~(\func{DirectProof}(\Left \models \Right)) ~ \Return ~\true \\
\\

     & {\bf let} ~\Left = \Phi, \LeftD_1, \ldots, \LeftD_n ~and~ \Right = \Psi, \RightD_1, \ldots, \RightD_m \\
\ppp & OrSet ~\Assign ~\emptyset \\


\ppp & \If ~(ib < {\sf INDUCTIONBOUND}) \ptab \ptab \mbox{/* Induction Application */} \\
% & \ptab \mbox{/* Abstract the LHS */} \\
\ppp     & \ptab \Foreach (\pair{p(\tilde{y}) \wedge \Left' \models \Right')}{p(\tilde{y})} \in \tilde{A}) \\
\ppp     & \ptab \ptab \func{Find} ~ p(\tilde{x}) \in \Left \mbox { s.t. } {\tt gen}(p(\tilde{x})) \geq {\tt kill}(p(\tilde{y})) \\
\ppp     & \ptab \ptab \func{Find} ~ \Left_1 \subseteq \Left \mbox{ s.t. } \theta ~\Assign ~\func{DirectProof}(\Left_1 \models \Left') ~\neq ~\perp \\
\ppp 	   & \ptab \ptab \If (\tilde{x} = \tilde{y}\theta ~and~\theta~ \mbox{is a valid renaming}) \\
\ppp 	   & \ptab \ptab \ptab \Left_{new} \Assign  \Left \setminus \{p(\tilde{x})\} \setminus  \Left_1 \cup \Right'\theta \\
\ppp     & \ptab \ptab \ptab OrSet ~\cup_{=} \{\afivetuple{\Left_{new} \models \Right}{\tilde{A}}{lb}{rb}{ib+1}\} \\
%\\
%     & \ptab \mbox{/* Strengthen the RHS */} \\
\ppp     & \ptab \Foreach (\pair{p(\tilde{y}) \wedge \Left' \models \Right')}{p(\tilde{y})} \in \tilde{A})\\
\ppp     & \ptab \ptab \If ~(\theta_1 ~\Assign ~\func{DirectProof}(\Right' \models \Right) = ~\perp) ~{\bf continue} \\
\ppp     & \ptab \ptab \func{Find} ~ p(\tilde{x}) \in \Left \mbox { s.t. } {\tt gen}(p(\tilde{x})) \geq {\tt kill}(p(\tilde{y})) \\
\ppp     & \ptab \ptab \func{Find} ~\mbox {a valid renaming } 
\theta \supseteq \theta_1 \mbox{ s.t. } \tilde{x} = \tilde{y}\theta \\
%\ppp & \ptab \ptab  \Left_1 ~\Assign ~\{\LeftD_i \in \Left ~|~ \func{stamp}(\LeftD_i) \geq 
%                                                 \func{stamp}(\Left' \models \Right')\} \\ 
%\ppp & \ptab \ptab  \func{Find} ~\emptyset \subset \Left'_1 \subseteq \Left', \theta \bullet 
%             ~\Left'_1 \theta \subseteq \Left_1 ~\&~\theta_1 \subseteq \theta \\
%\ppp & \ptab \ptab  \theta ~\Assign ~\func{merge}(\theta_1, \theta_2) \\
\ppp     & \ptab \ptab OrSet ~\cup_{=} \{\afivetuple{\Left \setminus \{p(\tilde{x})\} \models \Left'\theta}{\tilde{A}}{lb}{rb}{ib+1}\} \\
 %    & \Endif \\
\\




\ppp & \If ~(lb < {\sf MAXLEFTBOUND}) \ptab \ptab \mbox{/* Left Unfold */} \\


\ppp & \ptab \Foreach ~(\LeftD_i \in \Left) \\
\ppp & \ptab \ptab Obs ~\Assign  ~\emptyset \\
\ppp & \ptab \ptab \tilde{A}' ~\Assign ~\tilde{A} ~\cup ~\{\pair{\Left \models \Right}{\LeftD_i}\} \\
\ppp & \ptab \ptab \Foreach ~ (\Left_{j} \in (\{\Left_{1}, \Left_{2}, \ldots \Left_{l}\} ~\Assign ~{\sf UNFOLD}(\LeftD_i)))  \\

\ppp & \ptab \ptab \ptab ob ~\Assign 
    ~\afivetuple{(\Left_{j} \cup \Left \setminus \{\LeftD_i\}) \models \Right}{\tilde{A}'}{lb+1}{rb}{ib}\\
\ppp & \ptab \ptab \ptab \If ~ (\func{trivially\_true}(ob)) ~{\bf continue} \\
\ppp & \ptab \ptab \ptab Obs ~\Assign ~ Obs \cup \{ob\} \\
%     & \ptab \ptab \Endfor\\
\ppp & \ptab \ptab \If ~(Obs = ~\emptyset) ~\Return ~\true ~\Else ~OrSet ~\cup{=} ~\{Obs\} \\
 %    & \ptab \Endfor \\
%     & \Endif \\

\\
\ppp & \If ~(rb < {\sf MAXRIGHTBOUND} ~and ~ \neg \func{contradict}(\Left \models \Right)) \\
& \ptab \ptab  \mbox{/* Right Unfold */} \\

\ppp & \ptab \Foreach ~(\RightD_i \in \Right) \\
\ppp & \ptab \ptab \Foreach (~\Right_{j} \in \{\Right_{1}, \Right_{2}, \ldots \Right_{k}\} ~\Assign ~{\sf UNFOLD}(\RightD_i)) \\
\ppp & \ptab \ptab \ptab ob = \afivetuple{\Left \models (\Right_{j} \cup \Right \setminus \{\RightD_i\})}{\tilde{A}}{lb}{rb+1}{ib} \\
%\ppp & \ptab \ptab \ptab \If ~(\func{trivial\_false}(ob))~{\bf continue} \\
\ppp & \ptab \ptab \ptab OrSet ~\cup{=} \{\{ob\}\} \\
%     & \ptab \ptab \Endfor \\
%     & \ptab \Endfor \\
%     & \Endif \\
\\
\ppp & \If ~(OrSet ~= \emptyset) ~\Return ~\false \\
\ppp \label{algo:heuristics} & OrSet ~\Assign ~\func{OrderByHeuristics}(OrSet) \\
\ppp & \Foreach ~(Obs \in OrSet) \\
\ppp & \ptab \If ~(\func{ProveAll}(Obs)) ~\Return ~\true \\
%     & \Endfor \\
\ppp & \Return ~\false \\
\multicolumn{2}{l}{\mbox{\bf endfunction}}

\end{array}$
}
\vspace{-3mm}
\end{center}
\caption{The Algorithm\label{algm}}
\end{figure}


\begin{figure}[tbh]
\begin{center}
\small{
$\begin{array}{rl}

\multicolumn{2}{l}{\mbox{\bf function} ~\func{ProveAll}(Obs)}  \\
\ppp & \Foreach ~(\afivetuple{\Left \models \Right}{\tilde{A}}{lb}{rb}{ib} \in Obs) \\
\ppp & \ptab \If  ~(\neg ~\func{Prove}(\Left \models \Right, ~\tilde{A}, ~lb, ~rb, ~ib)) ~\Return ~\false; \\
%\ppp & \Endfor \\
\multicolumn{2}{l}{\mbox{\bf endfunction}} \\ 
\\


\multicolumn{2}{l}{\mbox{\bf function} ~\func{DirectProof}(\Left \models \Right)} \\
\ppp & \If ~(\exists ~q(\tilde{x}) \in \Right ~\mbox{such that} \not\exists ~q(\tilde{y}) \in \Left) 
          ~\Return ~ \perp \\
\ppp & \Left' ~\Assign  ~\func{get\_all\_recursive}(\Left) \\
\ppp & \Right' ~\Assign  ~\func{get\_all\_recursive}(\Right) \\
\ppp & \Theta ~\Assign ~\{\mbox{substitution}~ \theta ~|~ \Right'\theta \subseteq \Left' \} \\
\ppp & \If ~(\Theta ~= ~\emptyset) ~\Return ~\perp \\


\ppp & \Foreach ~(\theta  \in \Theta) \\
\ppp & \ptab \Phi ~\Assign ~\func{get\_all\_nonrecursive}(\Left) \\
\ppp & \ptab \Psi ~\Assign ~\func{get\_all\_nonrecursive}(\Right) \\
\ppp & \ptab \theta' ~\Assign ~\func{bind\_remaining\_existential\_variables}(\Psi, \Phi, \theta) \\
     & \ptab \mbox{/* Extend $\theta$ to $\theta'$ by trying obvious bindings} \\
     & \ptab \ptab \mbox{for remaining existential variables */}\\
\ppp & \ptab \If ~(\func{has\_existential\_variables}(\Psi, \Phi, \theta')) ~\bf{continue} \\
\ppp & \ptab \If ~(\func{entailment}(\Phi, \Psi \theta')) ~\Return ~\theta' \\
%     & \Endfor \\
\ppp & \Return ~\perp\\
\multicolumn{2}{l}{\mbox{\bf endfunction}}\\


\\
\multicolumn{2}{l}{\mbox{\bf function} ~\func{trivially\_true}(\afivetuple{\Left \models \Right}{\unknown}{\unknown}{\unknown}{\unknown})}  \\
\ppp & \Phi ~\Assign ~\func{get\_all\_nonrecursive}(\Left) \\
\ppp & \If ~(\func{unsatisfiable}(\Phi)) ~\Return ~\true\\
\ppp & \Return ~\false\\
\multicolumn{2}{l}{\mbox{\bf endfunction}}\\

\\

\multicolumn{2}{l}{\mbox{\bf function} ~\func{contradict}(\Left \models \Right)}  \\
\ppp & \Phi ~\Assign ~\func{get\_all\_nonrecursive}(\Left) \\
\ppp & \Psi ~\Assign ~\func{get\_all\_nonrecursive}(\Right) \\
\ppp & \Return ~(\func{satisfiable}(\Phi) ~\mbox{and} ~ \func{unsatisfiable}(\Phi \wedge \Psi)) \\
 \multicolumn{2}{l}{\mbox{\bf endfunction}}


%\\
\end{array}$
}
\vspace{-3mm}
\end{center}
\caption{Supporting Functions\label{algm}}
\end{figure}


\noindent
We now describe a systematic algorithm for dispensing
a proof obligation $\Left \models \Right$ mechanically. 
The main algorithm is in Figure~\ref{algm}.
In the figure, we use $X~\cup{=} ~Y$ to denote
$X ~\Assign ~X \cup Y$.
 
We start off by calling the function $\func{Prove}$ with the 
original obligation $\Left \models \Right$, the set of assumptions
$\tilde{A}$ to be $\emptyset$, and all the counters $lb, rb, ib$ to be $0$.
The counters $lb, rb, ib$ are to keep track of, respectively,
how many left unfolds, right unfolds, and inductions have been
applied in this current path. These counters are to ensure 
that our algorithm terminates.


\ignore{
An unoptimized proof obligation usually can be partitioned into
a number of smaller and simpler (e.g. by eliminating redundant terms and variables) proof obligations. This step
is taken care of by calling the function $\func{partition}$.
If it succeeds, we should proceed
by proving all the sub-obligations returned by the function.
We assume that a simple implementation of $\func{partition}$ is standard.
}



 

\vspace{2mm}
\noindent
{\bf Base Case:}
The function \func{DirectProof}
acts as the base case of our recursive algorithm.
This function corresponds to the repetitive applications of the ({\sc sub})
rule and a successful query to an \smt{} solver, after treating 
all recursive predicates in the LHS as uninterpreted (({\sc cp})-rule).


Intuitively, \func{DirectProof} succeeds if the proof obligation
is simple ``enough'' such that a {\it proof by matching} can be achieved.
We note here that, our proof rules in Section~\ref{sec:proofrules} allow
other rules (e.g. ({\sc ru}) rule in Example~\ref{ex:sub-ru}) to interleave
with the ({\sc sub}) and ({\sc cp}) rules.
However, in our deterministic algorithm,
applications of ({\sc sub}) and ({\sc cp}) rules
are coupled together within the function \func{DirectProof}.


\ignore{
Our function \func{DirectProof} is similar to the process 
of performing formula abstraction and 
then submitting the final formula to an \smt{} solver. 
The main difference is that, in their restricted setting, finding the appropriate
substitution for existential variables in the RHS is ``deterministic''.
Here the task requires some amount of search. However,
the cost of this search is negligible, since the number of 
recursive terms appear in the proof obligation is small.
}

Let us examine the function \func{DirectProof}.
If there is a recursive predicate $q$ on the RHS, but not in the LHS,
the function returns immediately, indicating failure with $\perp$.
Otherwise, the function then proceeds by finding some (not exhaustive)
substitutions $\Theta$ such that with each $\theta \in \Theta$,
we can simultaneously remove all the recursive predicates on the
RHS. This process will remove most existential variables on the RHS,
since existential variables usually appear in some recursive predicates.

In case there remain some existential variables on the RHS,
we attempt to bind them with the obvious candidates on the LHS
(therefore extend $\theta$ to $\theta'$).
%
%Some trivial rules, but often work in practice, are given below.
%Here $t$ is an existential variable
%while $x, y$  are not, and $f$ is a functional relation.
%
%\begin{itemize}
%\item
%if ($y = f(x) \wedge t = f(s) \wedge x \leftarrow s$) ~then $~y \leftarrow t$
%
%
%\item
%if ($x = f(y) \wedge s = f(t) \wedge x \leftarrow s$) then $y \leftarrow t$ (we treat as if
%$f$ is an injective function)
%
%\end{itemize}
%
%\noindent
After this attempt, if the RHS contains no existential variables,
we then call an \smt{} solver for entailment check.
If the answer is yes, $\theta'$ is returned,
indicating that a direct proof has been achieved.


\vspace{2mm}
\noindent
{\bf Recursive Call:}
We collect all possible transformations of the current proof obligation,
using  ({\sc ia-1}), ({\sc ia-2}), ({\sc lu+i}),
({\sc ru}) rules, into a set of set of obligations $OrSet$. 
The current proof obligation can be successfully discharged
if there is {\em any} $Obs \in OrSet$ ($Obs$ itself is a set of proof obligations), where
we can discharge {\em every} proof obligation $ob \in Obs$.
The realizations of the proof rules in our algorithm are straightforward, except
for a few noteworthy points:

\begin{enumerate}
\item
Our induction applications will not exhaustively
search for all possible candidates. Instead, we only search
for some trivial renaming which meet the side conditions of the rules.

\item When we perform left unfold, an obligation which is trivially true,
i.e. the non-recursive part of the LHS is unsatisfiable,  
is immediately removed.

\item If the current obligation contains the LHS and RHS which
contradict each other, right unfold will be avoided. The proof
for this obligation can succeed only if there is no model satisfies the LHS 
(so only left unfolds are required).
%In practice, the chance for such success is slim.

\end{enumerate}





\noindent 
We proceed our search for proof in a depth first search (DFS) manner.
The order in which the sets of obligations $Obs \in OrSet$ are considered
might heavily affect the efficiency, but not the effectiveness,  
of our algorithm.
Such order is dictated by our heuristics, as the call
to function \func{OrderByHeuristics} (line~\ref{algo:heuristics}) indicates.


We now discuss our simple heuristics which governs the 
implementation of the function \func{OrderByHeuristics}.
Most of them are intuitive and directly follow from the fact that 
our base case is only reached  by a successful call 
to \func{DirectProof} function.

%We first start with the order of pass


We proceed by a number of passes. 
%Each pass will consider a distinct ordering criterion.
In each pass, we first order the obligations within each $Obs \in OrderSet$.
We then consider the order of $OrderSet$ by comparing
the last obligation in each set $Obs \in OrderSet$.
Subsequent passes will not
undo the work of the previous passes, but instead will only
work on the obligations and/or sets of obligations which are tied in previous passes.


\begin{enumerate}
\item
An obligation which has contradicting LHS and RHS, given by the function $\func{contradict}$
will be ordered after those do not (since the chance to successfully
discharge such obligation is small).


\item
An obligation contains no recursive predicates on the RHS 
will be order before those contain some recursive predicate(s) on the RHS.

\item
An obligation having a recursive predicate $q$ such that $q$ appears
in the RHS but not in the LHS will be ordered after those not.

\item
An obligation contains more existential variables which cannot be
deterministically bound to some non-existential variables (variables on the LHS) will
be ordered after those contains less.

\item 
An obligation resulted from a left unfold will be ordered before 
those resulted from a right unfold (since it allows induction).


\end{enumerate}

\begin{example}
Revisit the obligation in Example~\ref{ex:sub-ru}:

\begin{center}
\stuff{
$\emptyset \vdash x \neq 0, list(x) \models \lseg(x,y), list(y)$.
}
%\qed
\end{center}
\end{example}

\noindent
For simplicity we ignore the information about the counters
$lb, rb,$ and $ib$.


First, the call to \func{DirectProof} fails since there is
the predicate $\lseg$ which appears in the RHS but not in
the LHS. Inductions do not take place either, as the set
of assumptions is currently empty.

We perform left unfold first. There is only one recursive predicate on the LHS.
Let $\tilde{A}'$ be \\
\indent 
$\{\pair{x \neq 0, list(x) \models \lseg(x,y), list(y)}{list(x)}\}$.

\noindent
The obligation \\
\indent
$\tilde{A}' \vdash x \neq 0, x = 0 \models \lseg(x,y), list(y)$

\noindent
is immediately discharged since the LHS is unsatisfiable.
We then end up with a set of one obligation, as the result for our left unfold:\\
\indent
$O_0 \equiv \{\tilde{A}' \vdash x \neq 0, z = x{\cdot}\nextpointer{}, list(z) \models \lseg(x,y), list(y)\}$ 

\noindent
We proceed with right unfold, producing four sets, each consists of one obligation as follows:

\begin{center}
\small{
\stuff{
$O_1 \equiv \{\emptyset \vdash x \neq 0, list(x) \models \lseg(x,y), y = 0\}$ \\
$O_2 \equiv \{\emptyset \vdash x \neq 0, list(x) \models \lseg(x,y), y \neq 0, z = y{\cdot}\nextpointer{}, list(z)\}$ \\
$O_3 \equiv \{\emptyset \vdash x \neq 0, list(x) \models x = y, list(y)\}$ \\
$ O_4 \equiv\{\emptyset \vdash x \neq 0, list(x) \models t \neq 0, y = t{\cdot}\nextpointer{}, \lseg(x,t), list(y)\}$
}
}
\end{center}

Assume that the initial order of those singleton sets of obligations are as shown above.
After the first two passes, the order between those singleton sets is the same.
The third pass, however, moves the singleton set $O_3$
to the first position. The fourth pass, on the other hand, moves 
$O_1$ to the second position.
The fifth pass keep $O_0$
at the third position. The remaining two  singleton sets,
namely $O_2$ and $O_4$
are tied and placed at the end.

We also comment that by proceeding with the first singleton
obligation set, namely $\{\emptyset \vdash x \neq 0, list(x) \models x = y, list(y)\}$,
a direct proof of it is successful. Therefore the original obligation is discharged successfully.
The corresponding sequence of applications of  proof rules is shown below,
which is slightly different from what shown in Section~\ref{sec:proofrules}. 


$$
\begin{array}{c}

\emptyset \vdash x \neq 0, list(x) \models \lseg(x,y), list(y) \\

 \mbox{\sc (ru)} \line(1,0){180} \\

\emptyset \vdash x \neq 0, list(x) \models x = y, list(y) \\
 
\mbox{\sc (sub)} \line(1,0){160} \\

\emptyset \vdash x \neq 0, list(x) \models x = x \\
 
\mbox{\sc (cp)}  \line(1,0){140} \\

\texttt{True}


\end{array}
$$





















